Recoverable Mutual Exclusion with Abortability

Recent advances in non-volatile main memory (NVRAM) technology have spurred research on designing algorithms that are resilient to process crashes. This paper is a fuller version of our conference paper \cite{jayanti:rmeabort}, which presents the first Recoverable Mutual Exclusion (RME) algorithm that supports abortability. Our algorithm uses only the read, write, and CAS operations, which are commonly supported by multiprocessors. It satisfies FCFS and other standard properties. Our algorithm is also adaptive. On DSM and Relaxed-CC multiprocessors, a process incurs $O(\min(k, \log n))$ RMRs in a passage and $O(f+ \min(k, \log n))$ RMRs in an attempt, where $n$ is the number of processes that the algorithm is designed for, $k$ is the point contention of the passage or the attempt, and $f$ is the number of times that $p$ crashes during the attempt. On a Strict CC multiprocessor, the passage and attempt complexities are $O(n)$ and $O(f+n)$. Attiya et al. proved that, with any mutual exclusion algorithm, a process incurs at least $\Omega(\log n)$ RMRs in a passage, if the algorithm uses only the read, write, and CAS operations \cite{Attiya:lbound}. This lower bound implies that the worst-case RMR complexity of our algorithm is optimal for the DSM and Relaxed CC multiprocessors.

==> invariant.tex <==
\newcommand{\invcond}[1]{\ref{inv:abrt:cond#1}}
\newcommand{\ih}{IH}
\newcommand{\indhyp}[1]{\mbox{\ih:\invcond{#1}}}
\newcommand{\casnormal}{CAS}

\begin{lemma}
	The algorithm in Figure~\ref{algo:abrt} satisfies the invariant (i.e., the conjunction of all the conditions)
	stated in Figure~\ref{inv:abrt}, i.e., the invariant holds in every configuration of every run of the algorithm.
\end{lemma}
\begin{proof} 
	 By induction. 
	
	For the base case, we verify that the conditions hold 
	in the initial configuration $C_0$ of any run.
	Condition~\invcond{1} holds in $C_0$ because $\token$ is initialized to $1$.
	Condition~\invcond{2} holds in $C_0$ because $\seq$ is initialized to $1$ and $\csowner$ is initialized to $(0,1)$.
	Condition~\invcond{5} holds in $C_0$ because $\pcp$ is initialized to \refln{abrt:rem:1}, $\go[p]$ to $-1$, and $\status_p$ to $\good$.
	Condition~\invcond{6} holds in $C_0$ because $\minarray[p]$ is initialized to $(p, \infty)$ and $\pcp$ is initially \refln{abrt:rem:1}.
	Condition~\invcond{7} holds in $C_0$ because initially $\pcp = \refln{abrt:rem:1}$, $\go[p] = -1$, and $\csowner = (0,1)$.
	Conditions~\invcond{8} through \invcond{13} hold trivially because $\pcp = \refln{abrt:rem:1}$ initially.
	Conditions~\invcond{3} and \invcond{4} also hold because the $\minarray$ is empty and $\csowner = (0, 1)$ initially.
	
	For the induction step, let $C$ be an arbitrary configuration of an arbitrary run.
	The induction hypothesis states that Conditions~\invcond{1} through \invcond{4} hold in $C$.
	Let $(C, \sigma, C')$ be an arbitrary (normal or crash) step of a process in $\procset$.
	We now establish the induction step by arguing that each of Conditions~\invcond{1} through \invcond{4} holds in $C'$.
	
	We use the following notation in the proof: (i) \ih\ denotes the induction hypothesis and, for all $i \in [\invcond{1}, \invcond{4}]$, 
	\ih:$i$ is the part of \ih\ that states that Condition $i$ of the invariant holds in $C$, and
	(ii) If $D$ is any configuration and $x$ is any variable, $D.x$ is the value of $x$ in $D$.
	
	\begin{enumerate}
		\item
		\underline{Proof that Condition \invcond{1} holds in $C'$}
		
		$\token$ changes only when a process $p$ executes Line~\refln{abrt:try:2}.
		If the \casnormal\ operation at that line succeeds, $\token$ increases by $1$; otherwise, it remains unchanged.
		Therefore, $C'.\token \ge C.\token$.
		Since $C.\token \ge 1$ by \indhyp{1}, we have $C'.\token \ge 1$.
		Thus, Condition~\invcond{1} holds in $C'$.
		
		\item
		\underline{Proof that Condition~\invcond{2} holds in $C'$}
		
		\begin{enumerate}
			\item
			Lines~\refln{abrt:exit:4} and \refln{abrt:prom:3} are the only lines of code that affect $\csowner$.
			
			\item
			If $\pcp = \refln{abrt:exit:4}$, \indhyp{8} implies that $C.\myseqp = C.\seq-1$.
			So, if a process $p$ writes $(0, \myseqp+1)$ in $\csowner$ at Line~\refln{abrt:exit:4}, Condition~\invcond{2} holds in $C'$.
			
			\item
			If $\pcp = \refln{abrt:prom:3}$ and $p$ executes a successful \casnormal\ to change $\csowner$ to $(1, \peerp)$,
			\indhyp{8} implies that $C.\peerp \in \procset$.
			So, Condition~\invcond{2} holds in $C'$.
		\end{enumerate}
		
		\item
		\underline{Proof that Condition~\invcond{5} holds in $C'$}
		
		We establish each of the conjuncts of Condition~\invcond{5}.
		
		\begin{enumerate}
			\item
			\underline{$-1 \le C'.\go[p] < \token$}
			
			We prove this statement through the following observations.
			
			\begin{enumerate}
				\item
				Lines~\refln{abrt:try:3}, \refln{abrt:exit:6}, \refln{abrt:abort:4}, and \refln{abrt:prom:6} are the only lines of code that affect $\go[p]$.
				
				\item
				If $\pcp = \refln{abrt:try:3}$, \indhyp{8} implies that $1 \le C.\tokp < \token$.
				So, if $p$ executes Line~\refln{abrt:try:3}, $-1 \le \go[p] < \token$ holds in $C'$.
				
				\item
				If $p$ executes Line~\refln{abrt:exit:6} or \refln{abrt:abort:4}, $\go[p]$ becomes $-1$, so $-1 \le \go[p] < \token$ holds in $C'$.
				
				\item
				If some  $q \in \procset$ performs a successful \casnormal\ at Line~\refln{abrt:prom:6} and $\peer{q} = p$, $\go[p]$ becomes $0$.
				Furthermore, \indhyp{1} implies that $0 < C.\token$.
				So, $-1 \le \go[p] < \token$ holds in $C'$.
			\end{enumerate}
			
			\item
			\underline{$C'.\pcp = \refln{abrt:try:4} \limplies C'.\go[p] = C'.\tokp$}
			
			To prove this implication, assume that $C'.\pcp = \refln{abrt:try:4}$. \\
			\\
			In case $C.\pcp = \refln{abrt:try:4}$, by \indhyp{5} $C.\go[p] = \tokp$ and the step from $C$ to $C'$ is by some $q \neq p$.
			If $q$ executes Line~\refln{abrt:prom:6} with $\peer{q} = p$, $\go[p]$ remains unchanged 
			because by \indhyp{13}, $\mygo{q} < \go[p]$ and hence the \casnormal\ by $p$ will fail.
			if $q$ executes any other line or executes a crash step, $\go[p]$ remains unchanged.
			Therefore, $C'.\go[p] = C.\go[p]$.\\
			\\
			In case $C.\pcp = \refln{abrt:try:3}$, $p$ sets $\go[p]$ to $\tokp$ at Line~\refln{abrt:try:3}, we have $C'.\go[p] = \tokp$.
			
			\item
			\underline{$C'.\pcp \in [ \refln{abrt:try:5}, \refln{abrt:try:7} ] \limplies C'.\go[p] \in \{0, C'.\tokp\}$}
			
			To prove this implication, assume that $C'.\pcp \in [ \refln{abrt:try:5}, \refln{abrt:try:7} ]$.
			We consider two cases:
			(i) $C.\pcp \not \in [ \refln{abrt:try:5}, \refln{abrt:try:7} ]$, or
			(ii) $C.\pcp \in [ \refln{abrt:try:5}, \refln{abrt:try:7} ]$.
			
			In Case (i), the step from $C$ to $C'$ must be $p$'s execution of Line~\refln{abrt:try:4}.
			By \indhyp{5} $C.\go[p] = \tokp$ and the step doesn't change the value of $\go[p]$, we have $C'.\go[p] = \tokp$.
			
			In Case (ii), we make two observations:
			
			\begin{enumerate}
				\item
				$C.\go[p] \in \{0, \tokp\}$ (by \indhyp{5}).
				\item
				$C'.\go[p] \in \{0, C.\go[p]\}$, as argued below. 
				
				\vspace{0.06in}
				If the step from $C$ to $C'$ is by $p$, it must be an execution of one of Lines~\refln{abrt:try:5}, \resolve{abrt:try:5}{abrt:prom:1} \upto \resolve{abrt:try:5}{abrt:prom:5}, or \refln{abrt:try:6}.
				Since $p$ does not change $\go[p]$ at these lines, $C'.\go[p] = C.\go[p]$.
				$\go[p]$ has the same value in $C'$ as it does in $C$.
				
				\vspace{0.06in}
				If the step from $C$ to $C'$ is by some $q$ and $q$ executes Line~\refln{abrt:prom:6}, $\go[p]$ either remains unchanged or changes to 0;
				if $q$ executes any other line or executes a crash step, $\go[p]$ remains unchanged.
				Therefore, $C'.\go[p] \in \{0, C.\go[p]\}$.
			\end{enumerate}
			
			It is immediate from the above two observations that $C'.\go[p] \in \{0, \tokp\}$.
			
			\vspace{0.09in}
			\item
			\underline{$C'.\pcp \in \{ \refln{abrt:try:8} \upto \refln{abrt:exit:6}, \refln{abrt:rec:2} \upto \refln{abrt:abort:4}, \refln{abrt:prom:1} \upto \refln{abrt:prom:6} \} \limplies C'.\go[p] \neq -1$}:
			
			To prove this implication, assume that in $C'.\pcp \in \{ \refln{abrt:try:8} \upto \refln{abrt:exit:6}, \refln{abrt:rec:2} \upto \refln{abrt:abort:4}, \refln{abrt:prom:1} \upto \refln{abrt:prom:6} \}$.
			We consider two cases: 
			(i) $C.\pcp \not \in \{ \refln{abrt:try:8} \upto \refln{abrt:exit:6}, \refln{abrt:rec:2} \upto \refln{abrt:abort:4}, \refln{abrt:prom:1} \upto \refln{abrt:prom:6} \}$, or
			(ii)  $C.\pcp \in \{ \refln{abrt:try:8} \upto \refln{abrt:exit:6}, \refln{abrt:rec:2} \upto \refln{abrt:abort:4}, \refln{abrt:prom:1} \upto \refln{abrt:prom:6} \}$.
			
			In Case (i), the step from $C$ to $C'$ must be $p$'s execution of Line~\refln{abrt:try:7}
			or of Line~\refln{abrt:rec:1} such that the step causes $\pcp$ to become \refln{abrt:rec:2}, or 
			$p$'s calling of $\promotep()$ at one of Lines \refln{abrt:try:5}, \refln{abrt:exit:5}, or \refln{abrt:abort:2}, which causes $\pcp$ to become \refln{abrt:prom:1}.
			We now consider each of these possibilities.
			
			\begin{enumerate}
				\item
				If $p$ executes Line~\refln{abrt:try:7}, it does not change $\go[p]$, so $C'.\go[p] = C.\go[p]$.
				Furthermore, \indhyp{5} implies $C.\go[p] \in \{0, \tokp\}$ and \indhyp{8} implies that $C.\tokp \neq -1$.
				Hence, $C'.\go[p] \neq -1$.
				\item
				If $p$ executes Line~\refln{abrt:rec:1} such that $C'.\pcp = \refln{abrt:rec:2}$,
				the instruction at Line~\refln{abrt:rec:1} implies that $C'.\go[p] \neq -1$.
				\item
				If $p$ calls $\promotep()$ at Line~\refln{abrt:try:5}, \indhyp{5} implies that $C.\go[p] \in \{0, \tokp\}$ and \indhyp{8} implies that $C.\tokp \neq -1$.
				Hence, $C'.\go[p] \neq -1$.
				\item
				If $p$ calls $\promotep()$ at Line~\refln{abrt:exit:5} or Line~\refln{abrt:abort:2}, \indhyp{5} implies that $C.\go[p] \neq -1$.
				Hence, $C'.\go[p] \neq -1$.
			\end{enumerate}
			
			Turning now to  Case (ii), we make the following observations:
			\begin{enumerate}
				\item
				$C.\go[p] \neq -1$ (by \indhyp{5}).
				\item
				$C'.\go[p] \in \{0, C.\go[p]\}$, as argued below. 
				
				\vspace{0.06in}
				If the step from $C$ to $C'$ is by $p$, since
				$\pcp \in \{ \refln{abrt:try:8} \upto \refln{abrt:exit:6}, \refln{abrt:rec:2} \upto \refln{abrt:abort:4}, \refln{abrt:prom:1} \upto \refln{abrt:prom:6} \}$ in both $C$ and $C'$,
				the step must be an execution of one of Lines~\refln{abrt:try:8}\upto\refln{abrt:exit:5},
				\refln{abrt:rec:2} \upto \refln{abrt:abort:3}, or  \refln{abrt:prom:1} \upto \refln{abrt:prom:6}.
				These lines, with the exception of Line~\refln{abrt:prom:6}, do not change $\go[p]$;
				and Line~\refln{abrt:prom:6}, if it changes $\go[p]$, sets it to 0.
				Therefore, $C'.\go[p] \in \{0, C.\go[p]\}$.
				
				\vspace{0.06in}
				If the step from $C$ to $C'$ is by some $q \neq p$,
				if $q$ executes Line~\refln{abrt:prom:6}, $\go[p]$ either remains unchanged or changes to 0;
				if $q$ executes any other line or executes a crash step, $\go[p]$ remains unchanged.
				Therefore, $C'.\go[p] \in \{0, C.\go[p]\}$.
			\end{enumerate}
			
			It is immediate from the above two observations that $C'.\go[p] \neq -1$.
			
			\item
			\underline{$(C'.\pcp \in \{ \refln{abrt:try:1} \upto \refln{abrt:try:3}, \refln{abrt:abort:5}  \} \vee (C'.\pcp \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge C'.\status_p \in \{ \good, \recrem \}))$ $\limplies$} \\
			\hspace*{3mm} \underline{$C'.\go[p] = -1$}
			
			We prove this implication in two parts.
			
			\begin{enumerate}
				\item
				\underline{$C'.\pcp \in \{ \refln{abrt:try:1} \upto \refln{abrt:try:3}, \refln{abrt:abort:5}  \} \limplies C'.\go[p] = -1$}
				
				Assume that $C'.\pcp \in \{ \refln{abrt:try:1} \upto \refln{abrt:try:3}, \refln{abrt:abort:5}  \} $.
				Then, there are the following three subcases to analyze. 
				
				\vspace{0.09in}
				\underline{Subcase A}: 
				Either $C.\pcp = \refln{abrt:rem:1} \; \wedge \; C.\status_p = \good$ or $C.\pcp = \refln{abrt:abort:4}$, and 
				$p$ executes a normal step.
				
				\vspace{0.09in}
				In this subcase, if $C.\pcp = \refln{abrt:rem:1} \; \wedge \; C.\status_p = \good$, \indhyp{5} implies that $C.\go[p] = -1$, so $C'.\go[p] = -1$.
				In (A), if $C.\pcp = \refln{abrt:abort:4}$, $p$ sets $\go[p]$ to $-1$ in the step, so $C'.\go[p] = -1$.
				
				\vspace{0.09in}
				\underline{Subcase B}: 
				$C.\pcp \in \{ \refln{abrt:try:1} \upto \refln{abrt:try:3}, \refln{abrt:abort:5}  \} $ and $p$ executes Line~\refln{abrt:try:1} or \refln{abrt:try:2}.
				
				\vspace{0.09in}
				In this subcase, \indhyp{5} implies that $C.\go[p] = -1$ and $p$'s step does not affect $\go[p]$, so $C'.\go[p] = -1$.
				
				\vspace{0.09in}
				\underline{Subcase C}: 
				$C.\pcp \in \{ \refln{abrt:try:1} \upto \refln{abrt:try:3}, \refln{abrt:abort:5}  \} $ and
				some $q \neq p$ executes a (normal or crash) step.
				
				\vspace{0.09in}
				In this subcase, \indhyp{5} implies that $C.\go[p] = -1$.
				The only line of code by which $q$ can change $\go[p]$ is via a successful \casnormal\ at Line~\refln{abrt:prom:6}.
				However, \indhyp{12} implies that $C.\mygo{q} \ge 0$, so $C.\mygo{q} \neq C.\go[p]$.
				Therefore, $q$'s execution of Line~\refln{abrt:prom:6} cannot affect $\go[p]$.
				Hence, $C'.\go[p] = C.\go[p] = -1$.
				
				\vspace{0.09in}
				We conclude that 
				$\pcp \in \{ \refln{abrt:try:1} \upto \refln{abrt:try:3}, \refln{abrt:abort:5}  \} \limplies \go[p] = -1$.
				
				\vspace{0.09in}
				\item
				\underline{$(C'.\pcp \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge C'.\status_p \in \{ \good, \recrem \}) \limplies C'.\go[p] = -1$}
				
				Assume that $C'.\pcp \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge C'.\status_p \in \{ \good, \recrem \}$.
				Then, there are the following four subcases to analyze:
				
				\vspace{0.09in}
				\underline{Subcase A}: $C.\pcp \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge C.\status_p \in \{ \good, \recrem \}$ and
				some process $q \neq p$ executes a (normal or crash) step.
				
				\vspace{0.09in}
				In this case, \indhyp{5} implies that $C.\go[p] = -1$.
				The only line of code by which $q$ can change $\go[p]$ is via a successful \casnormal\ at Line~\refln{abrt:prom:6}.
				However, \indhyp{12} implies that $C.\mygo{q} \ge 0$, so $C.\mygo{q} \neq C.\go[p]$.
				Therefore, $q$'s execution of Line~\refln{abrt:prom:6} cannot affect $\go[p]$.
				Hence, $C'.\go[p] = C.\go[p] = -1$.
				
				\vspace{0.09in}
				\underline{Subcase B}: $C.\pcp$ is \refln{abrt:exit:6}, \refln{abrt:abort:5}, or \refln{abrt:rec:1} (and $\go[p] = -1$), and $p$ executes a normal step (causing
				$\pcp$ to become \refln{abrt:rem:1}).
				
				\vspace{0.09in}
				If $C.\pcp = \refln{abrt:exit:6}$ and $p$ executes a normal step, $p$ sets $\go[p]$ to $-1$, so $C'.\go[p] = -1$.
				
				\vspace{0.09in}
				If $C.\pcp = \refln{abrt:abort:5}$, \indhyp{5} implies that $C.\go[p] = -1$; if $p$ executes a normal step,
				$\go[p]$ remains unchanged.
				Hence, $C'.\go[p] = -1$.
				
				\vspace{0.09in}
				If $C.\pcp = \refln{abrt:rec:1}$, $C.\go[p] = -1$, and $p$ executes a normal step, it is immediate that $C'.\go[p] = -1$.
				
				\vspace{0.09in}
				\underline{Subcase C}: $C.\pcp = \refln{abrt:rem:1} \, \wedge \, C.\status_p \in \{\good, \recrem \}$ and 
				$p$ invokes $\recoverprocp()$ (causing $\pcp$ to become \refln{abrt:rec:1}).
				
				\vspace{0.09in}
				\indhyp{5} implies that $C.\go[p] = -1$. Since $p$'s invocation of $\recoverprocp()$ does not affect $\go[p]$,
				it follows that $C'.\go[p] = -1$.
				
				\vspace{0.09in}
				\underline{Subcase D}: 
				$C.\pcp = \refln{abrt:rec:1} \, \wedge \, C.\status_p \in \{\good, \recrem \}$ and $p$ executes a crash step (causing
				$\pcp$ to become \refln{abrt:rem:1} and $\status_p$ to become $\recrem$).
				
				\vspace{0.09in}
				\indhyp{5} implies that $C.\go[p] = -1$. Since $p$'s crash step does not affect $\go[p]$,
				it follows that $C'.\go[p] = -1$.
				
				\vspace{0.09in}
				We conclude that 
				$(C'.\pcp \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge C'.\status_p \in \{ \good, \recrem \}) \limplies C'.\go[p] = -1$.
			\end{enumerate}
			
			From (a), (b), (c), (d), and (e), we conclude that Condition~\invcond{5} holds in $C'$.
		\end{enumerate}
		
		\item
		\underline{Proof that Condition~\invcond{6} holds in $C'$}
		
		In the following, we establish each of the conjuncts of Condition~\invcond{6}.
		
		\begin{enumerate}
			\item
			\underline{$\exists t \in [1, C'.\token-1] \cup \{\infty\}, C'.\minarray[p] = (p,t)$}
			
			We observe that $\minarray[p]$ is changed only by $p$ and only at Lines~\refln{abrt:try:4}, \refln{abrt:exit:1}, and \refln{abrt:abort:1}.
			If $\pcp = \refln{abrt:try:4}$, $p$ writes $(p, \tokp)$ in $\minarray[p]$, and \indhyp{8} implies that $1 \le C.\tokp < C.\token$;
			and if $\pcp$ is \refln{abrt:exit:1} or \refln{abrt:abort:1}, $p$ writes $(p, \infty)$ in $\minarray[p]$.
			Since $C'.\token = C.\token$, we conclude that $\exists t \in [1, C'.\token-1] \cup \{\infty\}, C'.\minarray[p] = (p,t)$.
			
			\item
			\underline{$C'.\pcp \in [ \refln{abrt:try:5}, \refln{abrt:try:7} ] \limplies C'.\minarray[p] = (p, C'.\tokp))$}
			
			When $p$ executes Line~\refln{abrt:try:4}, causing $\pcp$ to become \refln{abrt:try:5}, it writes $(p, \tokp)$ in $\minarray[p]$.
			Furthermore, neither $\minarray[p]$ nor $\tokp$ is changed by $p$ at Lines \refln{abrt:try:5} and \refln{abrt:try:6},
			or by any other process at any line.
			Therefore, we have $C'.\pcp \in [ \refln{abrt:try:5}, \refln{abrt:try:7} ] \limplies \minarray[p] = (p, C'.\tokp)$.
			
			\item
			\underline{$(C'.\pcp \in \{\refln{abrt:try:4}, \refln{abrt:exit:2} \upto \refln{abrt:exit:6}, \refln{abrt:abort:2} \upto \refln{abrt:abort:4} \} \vee  C'.\go[p] = -1)$ $\limplies$ 
				$C'.\minarray[p] = (p, \infty)$}
			
			We prove this implication in two parts.
			
			\begin{enumerate}
				\item
				\underline{$C'.\pcp \in \{\refln{abrt:try:4}, \refln{abrt:exit:2} \upto \refln{abrt:exit:6}, \refln{abrt:abort:2} \upto \refln{abrt:abort:4} \} \limplies C'.\minarray[p] = (p, \infty)$}
				
				To prove this implication, assume $C'.\pcp \in \{\refln{abrt:try:4}, \refln{abrt:exit:2} \upto \refln{abrt:exit:6}, \refln{abrt:abort:2} \upto \refln{abrt:abort:4} \}$.
				There are the following two subcases to analyze.
				
				\vspace{0.09in}
				\underline{Subcase A}: Assume that $C.\pcp \not \in \{\refln{abrt:try:4}, \refln{abrt:exit:2} \upto \refln{abrt:exit:6}, \refln{abrt:abort:2} \upto \refln{abrt:abort:4} \}$
				
				In this subcase, the step from $C$ to $C'$ must be $p$'s execution of any of Lines \refln{abrt:try:3}, \refln{abrt:exit:1}, or \refln{abrt:abort:1}.
				If $p$ executes Line~\refln{abrt:try:3}, \indhyp{5} implies that $C.\go[p] = -1$, which together with \indhyp{6}, implies that
				$C.\minarray[p] = (p, \infty)$.
				Since $p$ does not change $\minarray[p]$ at Line~\refln{abrt:try:3}, we have $C'.\minarray[p] = C.\minarray[p] = (p, \infty)$.
				
				\vspace{0.09in}
				If $p$ executes Line \refln{abrt:exit:1} or \refln{abrt:abort:1}, since it writes $(p, \infty)$ in $\minarray[p]$ at these lines,
				we have $C'.\minarray[p] = (p, \infty)$.
				
				\vspace{0.09in}
				\underline{Subcase B}: Assume that $C.\pcp \in \{\refln{abrt:try:4}, \refln{abrt:exit:2} \upto \refln{abrt:exit:6}, \refln{abrt:abort:2} \upto \refln{abrt:abort:4} \}$
				
				In this subcase, since $p$ does not change $\minarray[p]$ at Lines \refln{abrt:exit:2} \upto \refln{abrt:exit:5}, and at Lines \refln{abrt:abort:2} and \refln{abrt:abort:3},
				and any $q \neq p$ does not change $\minarray[p]$ (regardless of $q$'s step, normal or crash),
				we have $C'.\minarray[p] = C.\minarray[p]$.
				Furthermore, we have $C.\minarray[p] = (p, \infty)$ by \indhyp{6}.
				It follows that $C'.\minarray[p] = (p, \infty)$.
				
				\item
				\underline{$C'.\go[p] = -1 \limplies C'.\minarray[p] = (p, \infty)$}
				
				To prove this implication, assume $C'.\go[p] = -1$.
				There are the following two subcases to analyze.
				
				\vspace{0.09in}
				\underline{Subcase A}: Assume that $C.\go[p] = -1$.
				
				In this subcase, \indhyp{6} implies that $C.\minarray[p] = (p, \infty)$.
				Furthermore, since $C.\go[p] = -1$, \indhyp{5} and \indhyp{8} implies that $C.\pcp \neq \refln{abrt:try:4}$,
				so the step from $C$ to $C'$ is not $p$'s execution of Line~\refln{abrt:try:4}.
				Since the execution of Line~\refln{abrt:try:4} by $p$ is the only way to write a non-$\infty$ value in $\minarray[p]$,
				it follows that $C'.\minarray[p] = (p, \infty)$.
				
				\vspace{0.09in}
				\underline{Subcase B}: Assume that $C.\go[p] \neq -1$.
				
				In this subcase, since $C.\go[p] \neq -1$ and $C'.\go[p] = -1$, it follows that
				the step from $C$ to $C'$ is $p$'s execution of Line~\refln{abrt:exit:6} or Line~\refln{abrt:abort:4}.
				Thus, $C.\pcp \in \{\refln{abrt:exit:6}, \refln{abrt:abort:4}\}$.
				It follows from \indhyp{6} that $C.\minarray[p] = (p, \infty)$.
				Furthermore, since Lines \refln{abrt:exit:6} and \refln{abrt:abort:4} don't affect $\minarray[p]$, 
				we have $C'.\minarray[p] = C.\minarray[p] = (p, \infty)$.
				
			\end{enumerate}
			
			From (a), (b), and (c), we conclude that Condition~\invcond{6} holds in $C'$.
		\end{enumerate}
		
		\item
		\underline{Proof that Condition~\invcond{7} holds in $C'$}
		
		We establish Condition~\invcond{7} in parts.
		
		\begin{enumerate}
			\item
			\underline{Prove $(C'.\pcp \in [\refln{abrt:try:5}, \refln{abrt:try:7}] \wedge C'.\go[p] = 0) \limplies C'.\csowner = (1, p)$}
			
			To prove this implication, assume that $C'.\pcp \in [\refln{abrt:try:5}, \refln{abrt:try:7}] \wedge C'.\go[p] = 0$.
			We consider the following cases.
			
			\begin{itemize}
				\item
				\underline{Case 1}: $C.\pcp \in [\refln{abrt:try:5}, \refln{abrt:try:7}] \wedge C.\go[p] = 0$
				
				In this case, \indhyp{7} implies that $C.\csowner = (1, p)$.
				The only lines of code that can potentially change $\csowner$ are Lines~\refln{abrt:exit:4} and \refln{abrt:prom:3}.
				However, since $C.\csowner = (1, p)$, if any process executes Line~\refln{abrt:prom:3} from $C$,
				the \casnormal\ instruction at that line fails and $\csowner$ remains unchanged.
				Since $C.\pcp \in [\refln{abrt:try:5}, \refln{abrt:try:7}]$, the step from $C$ to $C'$ cannot be
				$p$'s execution of Line~\refln{abrt:exit:4}.
				Since $C.\csowner = (1, p)$, we have $\csowner \neq (1,q)$ for any $q \neq p$.
				Then, \indhyp{7} implies that $\pc{q} \neq \refln{abrt:exit:4}$.
				So, the step from $C$ to $C'$ cannnot be $q$'s execution of Line~\refln{abrt:exit:4}.
				We conclude that $C'.\csowner = C.\csowner = (1,p)$.
				
				\item
				\underline{Case 2}: $C.\pcp \in [\refln{abrt:try:5}, \refln{abrt:try:7}] \wedge C.\go[p] \neq 0$
				
				Since $C.\go[p] \neq 0$ and $C'.\go[p] = 0$, the step from $C$ to $C'$ must be
				the successful execution of the \casnormal\ instruction at Line~\refln{abrt:prom:6} by some process $q$
				with $\peer{q} = p$, as Line~\refln{abrt:prom:6} is the only line of code where $0$ is written into a $\go$ variable.
				Then, \indhyp{13} implies that $C.\csowner = (1, p)$.
				Since $q$'s execution of Line~\refln{abrt:prom:6} does not affect $\csowner$,
				it follows that $C'.\csowner  = C.\csowner = (1, p)$.
				
				\item
				\underline{Case 3}: $C.\pcp \not \in [\refln{abrt:try:5}, \refln{abrt:try:7}]$
				
				Since $C.\pcp \not \in [\refln{abrt:try:5}, \refln{abrt:try:7}]$ and $C'.\pcp \in [\refln{abrt:try:5}, \refln{abrt:try:7}]$,
				the step from $C$ to $C'$ must be $p$'s execution of Line~\refln{abrt:try:4}.
				Thus, $C.\pcp = \refln{abrt:try:4}$.
				Then, \indhyp{5} implies that $C.\go[p] = \tokp$ and \indhyp{8} implies that $\tokp \ge 1$.
				It follows that $C.\go[p] \neq 0$.
				Since $p$'s execution of Line~\refln{abrt:try:4} does not modify $\go[p]$,
				it follows that $C'.\go[p] = C.\go[p] \neq 0$, contradicting our earlier assumption that $C'.\go[p] = 0$.
				We conclude that Case 3 does not arise.
			\end{itemize}
			
			\item
			\underline{Prove $C'.\pcp \in [ \refln{abrt:cs:1}, \refln{abrt:exit:4} ] \limplies C'.\csowner = (1, p))$}
			
			Assume that $C'.\pcp \in [ \refln{abrt:cs:1}, \refln{abrt:exit:4} ]$.
			There are two cases to analyze.
			
			\begin{itemize}
				\item
				\underline{Case 1}: $C.\pcp \not \in [ \refln{abrt:cs:1}, \refln{abrt:exit:4} ]$
				
				Since $\pcp \in [ \refln{abrt:cs:1}, \refln{abrt:exit:4} ]$ is false in $C$ and true in $C'$,
				the step from $C$ to $C'$ must be $p$'s execution of Line~\refln{abrt:try:7} with $\go[p] = 0$,
				or of Line~\refln{abrt:abort:3} with $\csowner = (1, p)$.
				In the former case, \indhyp{7} implies that $C.\csowner = (1,p)$.
				Since Lines \refln{abrt:try:7} and \refln{abrt:abort:3} do not modify $\csowner$, it follows that $C'.\csowner = C.\csowner = (1,p)$.
				
				\item
				\underline{Case 2}: $C.\pcp \in [ \refln{abrt:cs:1}, \refln{abrt:exit:4} ]$
				
				In this case, \indhyp{7} implies that $C.\csowner = (1, p)$.
				The only lines of code that can potentially change $\csowner$ are Lines \refln{abrt:exit:4} and \refln{abrt:prom:3}.
				However, since $C.\csowner = (1, p)$, if any process executes Line~\refln{abrt:prom:3} from $C$,
				the \casnormal\ instruction at that line fails and $\csowner$ remains unchanged.
				Since $C'.\pcp \in [ \refln{abrt:cs:1}, \refln{abrt:exit:4} ]$, the step from $C$ to $C'$ cannot be
				$p$'s execution of Line~\refln{abrt:exit:4}.
				Since $C.\csowner = (1, p)$, we have $\csowner \neq (1,q)$ for any $q \neq p$.
				Then, \indhyp{7} implies that $\pc{q} \neq \refln{abrt:exit:4}$.
				So, the step from $C$ to $C'$ cannnot be $q$'s execution of Line~\refln{abrt:exit:4}.
				We conclude that $C'.\csowner = C.\csowner = (1, p)$.
			\end{itemize}
			
			\item
			\underline{Prove $(C'.\status_p = \reccs) \limplies C'.\csowner = (1, p)$}
			
			Assume that $C'.\status_p = \reccs$.
			There are two cases to analyze.
			
			\begin{itemize}
				\item
				\underline{Case 1}: $C.\status_p \neq \reccs$
				
				Since $C.\status_p \neq \reccs$ and $C'.\status_p = \reccs$,
				it must be the case that $p$ is in CS (i.e., $C.\pcp = \refln{abrt:cs:1}$) in $C$ and 
				the step from $C$ to $C'$ must be $p$'s crash step.
				Then, \indhyp{7} implies that $C.\csowner = (1, p)$.
				Since $\csowner$ is a non-volatile variable, $C'.\csowner = (1, p)$.
				
				\item
				\underline{Case 2}: $C.\status_p = \reccs$
				
				In this case, \indhyp{7} implies that $C.\csowner = (1, p)$.
				The only lines of code that can potentially change $\csowner$ are Lines \refln{abrt:exit:4} and \refln{abrt:prom:3}.
				However, since $C.\csowner = (1, p)$, if any process executes Line~\refln{abrt:prom:3} from $C$,
				the \casnormal\ instruction at that line fails and $\csowner$ remains unchanged.
				Since $C.\status_p = \reccs$, \indhyp{8} implies that $C.\pcp \neq \refln{abrt:exit:4}$.
				Hence, the step from $C$ to $C'$ cannot be $p$'s execution of Line~\refln{abrt:exit:4}.
				Since $C.\csowner = (1, p)$, we have $\csowner \neq (1,q)$ for any $q \neq p$.
				Then, \indhyp{7} implies that $\pc{q} \neq \refln{abrt:exit:4}$.
				So, the step from $C$ to $C'$ cannnot be $q$'s execution of Line~\refln{abrt:exit:4}.
				We conclude that $C'.\csowner = C.\csowner = (1,p)$.
			\end{itemize}
			
			\item
			\underline{Prove $C'.\pcp \in  \{ \refln{abrt:try:4}, \refln{abrt:abort:4} \} \cup [ \refln{abrt:exit:5}, \refln{abrt:exit:6}] \limplies  C'.\csowner \neq (1, p)$}
			
			Assume that $C'.\pcp \in  \{ \refln{abrt:try:4}, \refln{abrt:abort:4} \} \cup [ \refln{abrt:exit:5}, \refln{abrt:exit:6}]$.
			There are two cass to analyze.
			
			\begin{itemize}
				\item
				\underline{Case 1: $C.\pcp \not \in  \{ \refln{abrt:try:4}, \refln{abrt:abort:4} \} \cup [ \refln{abrt:exit:5}, \refln{abrt:exit:6}]$}
				
				Since $\pcp \in  \{ \refln{abrt:try:4}, \refln{abrt:abort:4} \} \cup [ \refln{abrt:exit:5}, \refln{abrt:exit:6}]$
				is false in $C$ and true in $C'$,
				the step from $C$ to $C'$ must be $p$'s execution of Line~\refln{abrt:try:3}, Line~\refln{abrt:abort:3} (with $\csowner \neq (1,p)$), or Line~\refln{abrt:exit:4}.
				
				\vspace{0.09in}
				If $p$ executes Line~\refln{abrt:try:3}, \indhyp{5} implies that $C.\go[p] = -1$, which together with \indhyp{7} implies that
				$C.\csowner \neq (1,p)$.
				Since $p$ does not modify $\csowner$ at Line~\refln{abrt:try:3}, it follows that $C'.\csowner = C.\csowner \neq (1,p)$.
				
				\vspace{0.09in}
				If $p$ executes Line~\refln{abrt:abort:3} with $\csowner \neq (1,p)$, then it is trivially the case that $C'.\csowner \neq (1,p)$.
				
				\vspace{0.09in}
				If $p$ executes Line~\refln{abrt:exit:4}, $p$ writes $(0, \myseqp+1)$ in $\csowner$.
				Hence, $C'.\csowner \neq (1,p)$.
				
				\item
				\underline{Case 2: $C.\pcp \in  \{ \refln{abrt:try:4}, \refln{abrt:abort:4} \} \cup [ \refln{abrt:exit:5}, \refln{abrt:exit:6}]$}
				
				Since $C.\pcp \in  \{ \refln{abrt:try:4}, \refln{abrt:abort:4} \} \cup [ \refln{abrt:exit:5}, \refln{abrt:exit:6}]$,
				\indhyp{7} implies that $C.\csowner \neq (1,p)$.
				The only line of code that can potentially change $\csowner$'s value to $(1,p)$ is Line~\refln{abrt:prom:3}.
				For a process $q$ (possibly $q=p$) to execute a successful \casnormal\ at Line~\refln{abrt:prom:3}
				and change $\csowner$ to $(1,p)$, it must be the case that 
				$C.PC_q = \refln{abrt:prom:3}$, $\csowner = (0, s_q)$, and $\peer{q} = p$.
				Then, \indhyp{11} implies that $C.\pcp \in [\refln{abrt:try:5}, \refln{abrt:try:7}] \cup \{\refln{abrt:rec:2}-\refln{abrt:abort:2}, \resolve{abrt:abort:2}{abrt:prom:1}, \resolve{abrt:abort:2}{abrt:prom:2}, \resolve{abrt:abort:2}{abrt:prom:3}, \refln{abrt:rem:1}, \refln{abrt:rec:1} \}$.
				This set of values for $C.\pcp$ is incompatible with the case we are considering
				because $C.\pcp \in  \{ \refln{abrt:try:4}, \refln{abrt:abort:4} \} \cup [ \refln{abrt:exit:5}, \refln{abrt:exit:6}]$ 
				in the case we are considering.
				We conclude that the step from $C$ to $C'$ cannot change the value in $\csowner$ to $(1, p)$.
				Hence,  $C'.\csowner \neq (1,p)$.
			\end{itemize}
			
			\item
			\underline{Prove $C'.\go[p] = -1 \limplies C'.\csowner \neq (1, p)$}
			
			Assume that $C'.\go[p] = -1$. There are two cases to analyze.
			
			\begin{itemize}
				\item
				\underline{Case 1}: $C.\go[p] \neq -1$
				
				Since $\go[p]$ is -1 in $C'$ but not in $C$, 
				the step from $C$ to $C'$ must be $p$'s execution of Line~\refln{abrt:exit:6} or Line~\refln{abrt:abort:4}.
				Thus, $C.\pcp \in \{\refln{abrt:exit:6}, \refln{abrt:abort:4}\}$.
				Then, \indhyp{7} implies that $C.\csowner \neq (1, p)$.
				Since $p$ does not change $\csowner$ in Line \refln{abrt:exit:6} or \refln{abrt:abort:4}, it follows that 
				$C'.\csowner \neq (1, p) = C.\csowner \neq (1, p)$.
				
				\item
				\underline{Case 2}: $C.\go[p] = -1$
				
				Since $C.\go[p] = -1$, \indhyp{7} implies that $C.\csowner \neq (1, p)$.
				The only line of code that can potentially change $\csowner$'s value to $(1,p)$ is Line~\refln{abrt:prom:3}.
				For a process $q$ (possibly $q=p$) to execute a successful \casnormal\ at Line~\refln{abrt:prom:3}
				and change $\csowner$ to $(1,p)$, it must be the case that 
				$C.\pc{q} = \refln{abrt:prom:3}$, $\csowner = (0, \myseq{q})$, and $\peer{q} = p$.
				This, together with \indhyp{11} and $C.\go_p = -1$, 
				implies that $C.\pcp \in [\refln{abrt:try:5}, \refln{abrt:try:7}] \cup \{\refln{abrt:rec:2} \upto \refln{abrt:abort:2}, \resolve{abrt:abort:2}{abrt:prom:1}, \resolve{abrt:abort:2}{abrt:prom:2}, \resolve{abrt:abort:2}{abrt:prom:3} \}$.
				This set of values for $C.\pcp$'s is incompatible with the case we are considering
				because \indhyp{5}, together with $C.\go[p] = -1$, implies that $C.\pcp \in  \{ \refln{abrt:rem:1} \upto \refln{abrt:try:3}, \refln{abrt:rec:1}, \refln{abrt:abort:5} \}$.
				We conclude that the step from $C$ to $C'$ cannot change the value in $\csowner$ to $(1,p)$.
				Hence,  $C'.\csowner \neq (1,p)$.
			\end{itemize}
		\end{enumerate}
		
		\item
		\underline{Proof that Condition~\invcond{8} holds in $C'$}
		
		This condition mostly concerns local variables---variables that are modified only 
		when $p$ executes a line of code or a crash step.
		We establish the condition in parts.
		
		\begin{enumerate}
			\item
			\underline{Proof of $C'.\pcp = \refln{abrt:try:2} \limplies 1 \leq C'.\tokp \leq C'.\token$}
			
			If $C.\pcp \neq \refln{abrt:try:2}$, the step from $C$ to $C'$ must be $p$'s execution of Line~\refln{abrt:try:1}.
			Inspection of Line~\refln{abrt:try:1}, together with \indhyp{1}, implies that $1 \leq C'.\tokp \leq C'.\token$.
			
			\vspace{0.09in}
			On the other hand, if $C.\pcp = \refln{abrt:try:2}$, \indhyp{8} implies that $1 \leq C.\tokp \leq C.\token$.
			Since $\pcp = \refln{abrt:try:2}$ in both $C$ and $C'$, the only step from $C$ to $C'$
			that can affect the condition is the execution of Line~\refln{abrt:try:2} by some process $q \neq p$.
			However, $q$'s execution of Line~\refln{abrt:try:2} does not decrease $\token$'s value.
			It follows that, since $1 \leq \tokp \leq \token$ holds in $C$, it continues to hold in $C'$.
			
			
			\item
			\underline{Proof of $C'.\pcp \in [\refln{abrt:try:3}, \refln{abrt:try:7}] \limplies 1 \leq C'.\tokp < C'.\token$}
			
			Assume that $C'.\pcp \in [\refln{abrt:try:3}, \refln{abrt:try:7}]$.
			We consider two cases.
			
			\begin{itemize}
				\item
				\underline{Case 1: $\pcp \in [\refln{abrt:try:3}, \refln{abrt:try:7}]$ is false in $C$}
				
				Since $\pcp \in [\refln{abrt:try:3}, \refln{abrt:try:7}]$ is false in $C$ and true in $C$,
				the step from $C$ to $C'$ must be $p$'s execution of Line~\refln{abrt:try:2}.
				Thus, $C.\pcp = \refln{abrt:try:2}$ and \indhyp{8} implies that either $1 \le C.\tokp = C.\token$ or $1 \le C.\tokp < C.\token$.
				In the former case, $p$'s execution of Line~\refln{abrt:try:2} increments $\token$ by 1.
				Thus, in either case, we have $1 \le C'.\tokp < C'.\token$.
				
				\item
				\underline{Case 2: $\pcp \in [\refln{abrt:try:3}, \refln{abrt:try:7}]$ is true in $C$}
				
				Since $\pcp \in [\refln{abrt:try:3}, \refln{abrt:try:7}]$ is true in $C$,
				\indhyp{8} implies that $1 \le \tokp < \token$ holds in $C$.
				Since $\pcp \in [\refln{abrt:try:3}, \refln{abrt:try:7}]$ in $C$ and $C'$,
				if $p$ takes a step from $C$, it executes one of Lines \refln{abrt:try:3}, \refln{abrt:try:4}, \refln{abrt:try:5}, or \refln{abrt:try:6},
				which do not affect $\tokp$ or $\token$.
				If a process $q \neq p$ takes a step from $C$,
				it can possibly change $\token$ by executing Line~\refln{abrt:try:2}, but 
				the \casnormal\ instruction at Line~\refln{abrt:try:2} ensures that $\token$'s value does not decrease.
				Therefore, since $1 \le \tokp < \token$ holds in $C$, it continues to hold in $C'$.
			\end{itemize}
			
			\item
			\underline{Proof of $C'.\pcp = \refln{abrt:exit:3} \limplies C'.\myseqp = C'.\seq$}
			
			Assume that $C'.\pcp = \refln{abrt:exit:3}$.
			
			\vspace{0.09in}
			Suppose that $\pcp \neq \refln{abrt:exit:3}$ in $C$. Then, the step from $C$ must be $p$'s execution of Line~\refln{abrt:exit:2}.
			Hence, $\myseqp = \seq$ in $C'$.
			
			\vspace{0.09in}
			Suppose that $\pcp = \refln{abrt:exit:3}$ in $C$.
			Then, \indhyp{8} implies that $C.\myseqp = C.\seq$ and \indhyp{7} implies that $C.\csowner = (1,p)$.
			Since $\pcp = \refln{abrt:exit:3}$ in both $C$ and $C'$, 
			the process that takes the step from $C$ is some $q \neq p$.
			Since Line~\refln{abrt:exit:2} is the only line that changes $\seq$,
			if $q$ changes $\seq$ in its step from $C$, $C.\pc{q}$ must be \refln{abrt:exit:2}.
			Then, \indhyp{7} implies that $C.\csowner = (1,q)$, contradicting that $C.\csowner = (1,p)$.
			We conclude that $q$'s step does not change $\seq$.
			So, $\myseqp = \seq$, which holds in $C$, remains true in $C'$.
			
			\item
			\underline{Proof of $\pcp =\refln{abrt:exit:4} \limplies \myseqp = \seq - 1$}
			
			Assume that $C'.\pcp = \refln{abrt:exit:3}$.
			
			\vspace{0.09in}
			Suppose that $\pcp \neq \refln{abrt:exit:4}$ in $C$. Then, the step from $C$ must be $p$'s execution of Line~\refln{abrt:exit:3}.
			Hence, \indhyp{8} implies that $C.\seq = C.\myseqp$ and the increment of $\myseqp$ at Line~\refln{abrt:exit:3} ensures
			$\myseqp = \seq -1$ in $C'$.
			
			\vspace{0.09in}
			Suppose that $\pcp = \refln{abrt:exit:4}$ in $C$.
			Then, \indhyp{8} implies that $C.\myseqp = C.\seq-1$ and \indhyp{7} implies that $C.\csowner = (1,p)$.
			Since $\pcp = \refln{abrt:exit:4}$ in both $C$ and $C'$, 
			the process that takes the step from $C$ is some $q \neq p$.
			Since Line~\refln{abrt:exit:2} is the only line that changes $\seq$,
			if $q$ changes $\seq$ in its step from $C$, $C.\pc{q}$ must be \refln{abrt:exit:2}.
			Then, \indhyp{7} implies that $C.\csowner = (1,q)$, contradicting that $C.\csowner = (1,p)$.
			We conclude that $q$'s step does not change $\seq$.
			So, $\myseqp = \seq-1$, which holds in $C$, remains true in $C'$.
			
			\item
			\underline{Proof of $\pcp \in [\resolve{abrt:try:5}{abrt:prom:1}, \resolve{abrt:try:5}{abrt:prom:6}] \cup [\resolve{abrt:exit:5}{abrt:prom:1}, \resolve{abrt:exit:5}{abrt:prom:6}] \limplies \isabortingp = \false$}
			
			This statement follows from the observation that $\promote{}()$ is called at Line~\refln{abrt:try:5} and at Line~\refln{abrt:exit:5}
			with $\false$ as the parameter.
			
			\item
			\underline{Proof of $\pcp \in [\resolve{abrt:abort:2}{abrt:prom:1}, \resolve{abrt:abort:2}{abrt:prom:6}] \limplies \isabortingp = \true$}
			
			This statement follows from the observation that $\promote{}()$ is called at Line~\refln{abrt:abort:2}
			with $\true$ as the parameter.
			
			
			\item
			\underline{Proof of $\pcp \in [\refln{abrt:prom:3}, \refln{abrt:prom:6}] \limplies \peerp \in \procset$}
			
			This statement follows from the observation that, as $p$ enters Line~\refln{abrt:prom:3} from Line~\refln{abrt:prom:2},
			it sets $\peerp$ to either $p$ or the first component of the value it found in $\minarray[p]$.
			In either case, $\peerp \in \procset$.
			
			\item
			\underline{Proof of $C'.\pcp \in [\refln{abrt:try:1}, \refln{abrt:exit:6}] \limplies C'.\status_p = \good$}
			
			Assume that $C'.\pcp \in [\refln{abrt:try:1}, \refln{abrt:exit:6}]$.
			We consider two cases.
			
			\vspace{0.09in}
			Suppose that $C.\pcp \not \in [\refln{abrt:try:1}, \refln{abrt:exit:6}]$.
			Then, the step from $C$
			must be either $p$'s invocation of $\tryprocp()$ (from the remainder section of Line~\refln{abrt:rem:1}) 
			when $\status_p = \good$,
			or entry into the CS (Line~\refln{abrt:cs:1}) because $\recoverprocp()$ returns $\gotocs$ at Line~\refln{abrt:rec:2},
			simultaneously setting $\status_p$ to $\good$.
			In either case, we have $C'.\status_p = \good$.
			
			\vspace{0.09in}
			Suppose that $C.\pcp \in [\refln{abrt:try:1}, \refln{abrt:exit:6}]$.
			By \indhyp{8}, $C.\status_p = \good$.
			If $p$ takes a crash step from $C$, $\pcp$ becomes \refln{abrt:rec:1}, contradicting that $C'.\pcp \in [\refln{abrt:try:1}, \refln{abrt:exit:6}]$.
			If $p$ takes a normal step from $C$ or a different process takes a (normal or crash) step from $C$,
			$C'.\status_p = \good$ because $C.\status_p = \good$.
			
		\end{enumerate}
		
		\item
		\underline{Proof that Condition~\invcond{9} holds in $C'$}
		
		We prove this condition in two parts.
		
		\begin{enumerate}
			\item
			\underline{Proof of $C'.\pcp = \refln{abrt:try:7} \limplies (C'.\go[p] = 0 \vee \textnormal{abort was requested})$}
			
			Assume that $C'.\pcp = \refln{abrt:try:7}$.
			We consider two cases.
			
			\vspace{0.09in}
			Suppose that $C.\pcp \neq \refln{abrt:try:7}$.
			Then, the step from $C$ must be $p$'s read of 0 in $\go[p]$ or of $\true$ in $\abort[p]$ at Line~\refln{abrt:try:6}.
			Hence, we have $C'.\go[p] = 0 \vee \textnormal{abort was requested}$.
			
			\vspace{0.09in}
			Suppose that $C.\pcp = \refln{abrt:try:7}$.
			Then, \indhyp{9} implies that $C.\go[p] = 0 \vee \textnormal{abort was requested}$.
			Since $\pcp = \refln{abrt:try:7}$ in both $C$ and $C'$, the process that takes the step from $C$ 
			is some $q \neq p$.
			There is no line of code where $q$ can possibly change $\go[p]$ to any non-zero value.
			Therefore, the condition $\go[p] = 0 \vee \textnormal{abort was requested}$, which holds in $C$,
			continues to hold in $C'$.
			
			\item
			\underline{Proof of $C'.\pcp = \refln{abrt:try:8} \limplies \textnormal{abort was requested}$}
			
			When $\pcp = \refln{abrt:try:7}$, \indhyp{9} implies that $\go[p] = 0 \vee \textnormal{abort was requested}$.
			So, when $p$ executes the \ifcode statement at Line~\refln{abrt:try:7} and enters Line~\refln{abrt:try:8},
			$\textnormal{abort was requested}$ is true.
		\end{enumerate}
		
		\item
		\underline{Proof that Condition~\invcond{10} holds in $C'$}
		
		We prove this condition in parts.
		
		\begin{enumerate}
			\item
			\underline{Proof of $\pcp \in \{ \refln{abrt:prom:2}, \refln{abrt:prom:3} \} \limplies \myseqp \leq \seq$}
			
			Suppose that $p$ executes the step from $C$, and in the step,
			$p$ executes Line~\refln{abrt:prom:1} and enters Line~\refln{abrt:prom:2}.
			It follows that at Line~\refln{abrt:prom:1}, $p$ reads $(0, \myseqp)$ and, by \indhyp{2}, $\myseqp = C.\seq$.
			Since \indhyp{8} ensures that Line~\refln{abrt:exit:3} does not decrease the value of $\seq$,
			it follows that $\pcp \in \{ \refln{abrt:prom:2}, \refln{abrt:prom:3} \} \limplies \myseqp \leq \seq$.
			
			\item
			\underline{$\forall q \in \procset, (\pcp \in \{ \refln{abrt:prom:2}, \refln{abrt:prom:3} \} \wedge \pc{q} \in \{ \refln{abrt:exit:3}, \refln{abrt:exit:4} \}) \limplies \myseqp \leq \myseq{q}$}
			
			Assume that $C'.\pcp \in \{ \refln{abrt:prom:2}, \refln{abrt:prom:3} \} \wedge C'.\pc{q} \in \{ \refln{abrt:exit:3}, \refln{abrt:exit:4} \}$, for an arbitrary $q \in \procset$. We consider two cases.
			
			\begin{itemize}
				\item
				\underline{Case 1}: 
				The condition $\pcp \in \{ \refln{abrt:prom:2}, \refln{abrt:prom:3} \} \wedge  \pc{q} \in \{ \refln{abrt:exit:3}, \refln{abrt:exit:4} \}$ is false in $C$.
				
				Since the condition is true in $C'$, it must be the case that either
				$\pc{q} \in \{ \refln{abrt:exit:3}, \refln{abrt:exit:4} \}$ is true in $C$ and $p$ executes Line~\refln{abrt:prom:1} from $C$ (to enter Line~\refln{abrt:prom:2}), or
				$\pcp \in \{ \refln{abrt:prom:2}, \refln{abrt:prom:3} \}$ is true in $C$ and
				$q$ executes Line~\refln{abrt:exit:2} from $C$ (to enter Line~\refln{abrt:exit:3}).
				In the former case, \indhyp{7} implies that $C.\csowner = (1,q)$, so in its step from $C$,
				$p$ reads $(1,q)$ at Line~\refln{abrt:prom:1} and goes to Line~\refln{abrt:prom:4}, contradicting that $p$ moves to Line~\refln{abrt:prom:2}.
				In the latter case, $q$'s step from $C$ sets $\myseq{q}$ to $\seq$, and \indhyp{10} implies that $C.\myseqp \leq C.\seq$.
				Hence, we have $\myseqp \leq \myseq{q}$ in $C'$.
				
				\item
				\underline{Case 2}: 
				The condition $\pcp \in \{ \refln{abrt:prom:2}, \refln{abrt:prom:3} \} \wedge  \pc{q} \in \{ \refln{abrt:exit:3}, \refln{abrt:exit:4} \}$ is true in $C$.
				
				Since the condition is true in $C$, \indhyp{10} implies that $\myseqp \leq \myseq{q}$ is true in $C$.
				Furthermore, since the condition is true in both $C$ and $C'$, it follows that the step from $C$
				is $p$'s execution of Line~\refln{abrt:prom:2}, or $q$'s execution of Line~\refln{abrt:exit:3}, or an arbitrary step of a process
				different from $p$ and $q$.
				In all these cases, $\myseqp$ and $\myseq{q}$ are unaffected, so $\myseqp \leq \myseq{q}$ remains true in $C'$.
			\end{itemize}
		\end{enumerate}
		
		\item
		\underline{Proof that Condition~\invcond{11} holds in $C'$}
		
		We prove this condition in parts.
		
		\begin{enumerate}
			\item
			\underline{Assume $C'.\pcp = \refln{abrt:prom:2} \wedge C'.\csowner = (0, \myseqp)$.}
			
			Let $q$ be any process in $\procset$ (including possibly $p$),
			and assume that $C'.\minarray[q] \neq (q, \infty)$.
			Since $C'.\pcp = \refln{abrt:prom:2}$, $C.\pcp$ must be either \refln{abrt:prom:1} or \refln{abrt:prom:2}.
			We analyze these cases below and show that in each case, 
			$C'.\pc{q} \in \{\refln{abrt:try:5}-\refln{abrt:try:8}, \refln{abrt:rec:2}, \refln{abrt:abort:1} \}$ or $C'.\pc{q} \in \{\refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge C'.\go[q] \neq -1$.
			
			\begin{itemize}
				\item
				\underline{Case 1}: $C.\pcp = \refln{abrt:prom:1}$
				
				Since $\pcp$ is \refln{abrt:prom:1} in $C$ and \refln{abrt:prom:2} in $C'$, the step from $C$ to $C'$ must be $p$'s execution of Line~\refln{abrt:prom:1}, 
				where it finds $(0, \myseqp)$ in $\csowner$.
				Since Line~\refln{abrt:prom:1} does not change $\minarray$, we have
				$C.\minarray[q] = C'.\minarray[q] \neq (q, \infty)$.
				It follows from \indhyp{6} that $C.\pc{q} \not \in \{\refln{abrt:try:4}, \refln{abrt:exit:2}-\refln{abrt:exit:6}, \refln{abrt:abort:2}-\refln{abrt:abort:4}\}$ and $C.\go[q] \neq -1$.
				Furthermore, since $C.\csowner = (0, \myseqp) \neq (1,q)$, it follows from \indhyp{7} that
				$C.\pc{q} \not \in [\refln{abrt:cs:1}, \refln{abrt:exit:4}]$.
				Since $\go[q] \neq -1$, it follows from \indhyp{5} that $C.\pc{q} \not \in \{\refln{abrt:try:1} -\refln{abrt:try:3}, \refln{abrt:abort:5}\}$.
				Together, the above conditions imply $C.\pc{q} \in \{ \refln{abrt:try:5}-\refln{abrt:try:8}, \refln{abrt:rec:2}, \refln{abrt:abort:1}\}$ or $C.\pc{q} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge \go[q] \neq -1$.
				Regardless of whether $q=p$ or not, the same condition holds in $C'$, i.e.,
				$C'.\pc{q} \in \{ \refln{abrt:try:5}-\refln{abrt:try:8}, \refln{abrt:rec:2}, \refln{abrt:abort:1} \} \vee (C'.\pc{q} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge \go[q] \neq -1)$.
				
				\item
				\underline{Case 2}: $C.\pcp = \refln{abrt:prom:2} \wedge C.\csowner \neq (0, \myseqp)$
				
				In this case, since $C.\csowner \neq (0, \myseqp)$ and $C'.\csowner = (0, \myseqp)$,
				the step from $C$ must be the execution of Line~\refln{abrt:exit:4} by some process $r$.
				However, \indhyp{10} implies that $C.\myseqp \le C.\myseq{r}$.
				Since $r$ writes $(0, \myseq{r} + 1)$ in $\csowner$, it follows that $C'.\csowner \neq (0,\myseqp)$,
				contradicting our initial assumption.
				We conclude that Case 2 cannot arise.
				
				\item
				\underline{Case 3}: $C.\pcp = \refln{abrt:prom:2} \wedge C.\csowner = (0, \myseqp)$
				
				Suppose that $C.\minarray[q] = (q, \infty)$.
				Then, since $C'.\minarray[q] \neq (q, \infty)$,
				the step from $C$ must be $q$'s execution of Line~\refln{abrt:try:4}.
				Hence, $C'.\pc{q} = \refln{abrt:try:5}$.
				
				\vspace{0.09in}
				Next, suppose that $C.\minarray[q] \neq (q, \infty)$.
				Then, \indhyp{11} implies that 
				$C.\pc{q} \in \{ \refln{abrt:try:5}-\refln{abrt:try:8}, \refln{abrt:rec:2}, \refln{abrt:abort:1} \} \vee (C.\pc{q} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge C.\go[q] \neq -1)$.
				The only way that this condition becomes $\false$ in $C'$ is when $C.\pc{q} = \refln{abrt:abort:1}$
				and $q$ executes a step.
				However, $q$'s step causes $C'.\minarray[q]$ to be $(q, \infty)$, contradicting our assumption.
				
			\end{itemize}
			
			\item
			\underline{Assume $C'.\pcp = \refln{abrt:prom:3} \wedge C'.\csowner = (0, \myseqp)$}
			
			Since $C'.\pcp = \refln{abrt:prom:3}$, $C.\pcp$ must be either \refln{abrt:prom:2} or \refln{abrt:prom:3}.
			We analyze by cases below.
			
			
			\begin{itemize}
				\item
				\underline{Case 1}: $C.\pcp = \refln{abrt:prom:2}$
				
				Since $\pcp$ is \refln{abrt:prom:2} in $C$ and \refln{abrt:prom:3} in $C'$, the step from $C$ to $C'$ must be $p$'s execution of Line~\refln{abrt:prom:2}, 
				where $\findmin()$ returns $(\peerp, \tokp)$ and either $\tokp \neq \infty$ or $C.\isabortingp = \true$ and $C'.\peerp = p$. We consider each of these possibilities below.
				
				Suppose that $\findmin()$ returns $(\peerp, \tokp)$ and $\tokp \neq \infty$.
				This implies that $C.\minarray[\peerp] \neq (\peerp, \infty)$.
				It follows from \indhyp{11} that 
				$C.\pc{\peerp} \in \{ \refln{abrt:try:5}-\refln{abrt:try:8}, \refln{abrt:rec:2}, \refln{abrt:abort:1} \} \vee (C.\pc{\peerp} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge C.\go[\peerp] \neq -1)$.
				If $\peerp \neq p$, the same condition holds for $C'$.
				In $\peerp = p$, then the condition implies that $p$'s step from $C$ is the execution of Line~\refln{abrt:prom:2},
				as part of $\promotep()$ called from Line~\refln{abrt:try:5}, and the condition remains true for $C'$.
				Thus, we have $C'.\pc{\peerp} \in \{\refln{abrt:try:5}-\refln{abrt:try:8}, \refln{abrt:rec:2}, \refln{abrt:abort:1} \} \vee (C'.\pc{\peerp} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge C'.\go[\peerp] \neq -1)$.
				
				\vspace{0.09in}
				Next, suppose that $C.\isabortingp = \true$ and $C'.\peerp = p$.
				Then, $C'.\pc{\peerp} = C'.\pcp = \resolve{abrt:abort:2}{abrt:prom:3}$, and $\myseq{\peerp} = \myseqp$.
				
				\item
				\underline{Case 2}: $C.\pcp = \refln{abrt:prom:3} \wedge C.\csowner \neq (0, \myseqp)$
				
				In this case, since $C.\csowner \neq (0, \myseqp)$ and $C'.\csowner = (0, \myseqp)$,
				the step from $C$ must be the execution of Line~\refln{abrt:exit:4} by some process $r$.
				However, \indhyp{10} implies that $C.\myseqp \le C.\myseq{r}$.
				Since $r$ writes $(0, \myseq{r}+1)$ in $\csowner$, it follows that $C'.\csowner \neq (0, \myseqp)$,
				contradicting our initial assumption.
				We conclude that Case 2 cannot arise.
				
				\item
				\underline{Case 3}: $C.\pcp = \refln{abrt:prom:3} \wedge C.\csowner = (0, \myseqp)$
				
				\indhyp{11} implies that 
				$C.\pc{\peerp} \in \{\refln{abrt:try:5}-\refln{abrt:try:7}, \refln{abrt:rec:2}, \refln{abrt:abort:1}, \refln{abrt:abort:2}, \resolve{abrt:abort:2}{abrt:prom:1} \} \vee 
				(C.\pc{\peerp} \in \{ \resolve{abrt:abort:2}{abrt:prom:2}, \resolve{abrt:abort:2}{abrt:prom:3} \} \wedge \myseq{\peerp} = \myseqp) \vee
				(C.\pc{\peerp} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge C.\go[q] \neq -1)$.
				Even if $\peerp$ takes a step from $C$, this condition remains true in $C'$, as we explain below.
				
				\begin{itemize}
					\item
					Suppose that $\pc{\peerp}$ changes from \refln{abrt:try:7} in $C$ to \refln{abrt:cs:1} in $C'$.
					Then, \indhyp{7} implies that $C'.\csowner = (1, \peerp)$, which is impossible because
					$C.\csowner = (0, \myseqp)$ and the step from $C$ is the execution of Line~\refln{abrt:try:7}.
					
					\item
					Suppose that $\peerp$ takes a step from $C$ when $C.\pc{\peerp} = \resolve{abrt:abort:2}{abrt:prom:1}$.
					Since $C.\csowner = (0, \myseqp)$, it follows that $C'.\pc{\peerp} = \resolve{abrt:abort:2}{abrt:prom:2}$ and $C'.\myseq{\peerp} = C'.\myseqp$.
					
					\item
					Suppose that $\peerp$ takes a step from $C$ when $C.\pc{\peerp} = \resolve{abrt:abort:2}{abrt:prom:3}$.
					Then, since $C.\csowner = (0, \myseqp)$ and \indhyp{11} implies that $C.\myseq{\peerp} = C.\myseqp$,
					it follows that $C'.\csowner = (1, \peerp)$, contradicting our assumption that 
					$C'.\csowner = (0, \myseqp)$.
					
					\item
					Suppose that $\peerp$ takes a step from $C$ when $C.\pc{\peerp} = \refln{abrt:rem:1}$.
					Then, \indhyp{11} implies that $\go[\peerp] \neq -1$, which together with \indhyp{5} implies that 
					$\status_{\peerp} \neq \good$.
					It follows that, in its step from $C$, $\peerp$ invokes $\recoverproc{\peerp}()$ method;
					so, $C'.\pc{\peerp} = \refln{abrt:rec:1}$ (and $C'.\go[\peerp] \neq -1$).
				\end{itemize}
				
			\end{itemize}
		\end{enumerate}
		
		\item
		\underline{Proof that Condition~\invcond{12} holds in $C'$}
		
		Assume that $C'.\pcp \in \{ \refln{abrt:prom:5}, \refln{abrt:prom:6} \}$.
		We consider two cases.
		
		\begin{itemize}
			\item
			\underline{Case 1}: $C.\pcp \not \in \{\refln{abrt:prom:5}, \refln{abrt:prom:6} \}$
			
			Since $C.\pcp \not \in \{\refln{abrt:prom:5}, \refln{abrt:prom:6} \}$, the step from $C$ must be $p$'s execution of Line~\refln{abrt:prom:4} and
			$C'.\mygop = C.\go[\peerp] \not \in \{0, -1\}$.
			Since \indhyp{5} implies that $-1 \le C.\go[\peerp] < C.\token$,
			it follows that $1 \le C'.\mygop < C'.\token$.
			
			\item
			\underline{Case 2}: $C.\pcp \in \{\refln{abrt:prom:5}, \refln{abrt:prom:6}\}$
			
			In this case, \indhyp{12} implies that $1 \le \mygop < \token$ in $C$.
			Since $\token$ is possibly modified only at Line~\refln{abrt:try:2}, where the \casnormal\ instruction ensures that
			the value of $\token$ does not decrease, the inequality continues to hold in $C'$,
			i.e., $1 \le C'.\mygop < C'.\token$.
			
		\end{itemize}
		
		\item
		\underline{Proof that Condition~\invcond{13} holds in $C'$}
		
		Assume that $C'.\pcp = \refln{abrt:prom:6}$ and consider the following cases.
		
		\begin{itemize}
			\item
			\underline{Case 1}: $C.\pcp \neq \refln{abrt:prom:6}$
			
			Since $\pcp$ is \refln{abrt:prom:6} in $C'$ but not in $C$, it follows that
			the step from $C$ must be $p$'s execution of Line~\refln{abrt:prom:5} and $C.\csowner = (1,\peerp)$.
			\indhyp{7}, together with $C.\csowner = (1,\peerp)$, implies that
			$C.\pc{\peerp} \not \in \{\refln{abrt:try:4}, \refln{abrt:abort:4}\} \cup [\refln{abrt:exit:5}, \refln{abrt:exit:6}]$ and $C.\go[\peerp] \neq -1$.
			\indhyp{5}, together with $C.\go[\peerp] \neq -1$, implies that
			$\pc{\peerp} \not \in \{ \refln{abrt:try:1} \upto \refln{abrt:try:3}, \refln{abrt:abort:5}\}$.
			Taken together, the above facts imply that $C'.\pc{\peerp} \not \in \{ \refln{abrt:try:2}, \refln{abrt:try:3}, \refln{abrt:try:4} \}$.
			This, together with $C'.\csowner = C.\csowner = (1, \peerp)$,
			trivially implies Condition~\invcond{13} in $C'$.
			
			\underline{Case 2}: $C.\pcp = \refln{abrt:prom:6}$
			
			In this case, by the induction hypothesis, the consequent of Condition~\invcond{13}'s implication holds in $C$.
			We argue below that a step from $C$ cannot invalidate the consequent.
			
			\begin{itemize}
				\item
				Suppose that $\peerp$ takes a step from $C$ when $C.\pc{\peerp} = \refln{abrt:try:1}$.
				Then, $\pc{\peerp}$ becomes \refln{abrt:try:2} in $C'$,
				but then $1 \le \mygop < \tok{\peerp}$ will hold in $C'$
				because $\peerp$'s execution of Line~\refln{abrt:try:1} sets $\tok{\peerp}$ to $\token$,
				and \indhyp{12} implies that $1 \le \mygop < \token$.
				
				\item
				Suppose that $\peerp$ takes a step from $C$ when $C.\pc{\peerp} = \refln{abrt:try:3}$.
				Then, $\pc{\peerp}$ becomes \refln{abrt:try:4} in $C'$,
				but then $1 \le \mygop < \go[\peerp]$ will hold in $C'$
				because $\peerp$'s execution of Line~\refln{abrt:try:3} sets $\go[\peerp]$ to $\tok{\peerp}$,
				while \indhyp{13} and \indhyp{8} imply $1 \le \mygop < \tok{\peerp} < \token$.
				
				\item
				Suppose that $\peerp$ takes a step from $C$ when $C.\pc{\peerp} = \refln{abrt:try:4}$.
				Then, $\pc{\peerp}$ becomes \refln{abrt:try:5} in $C'$,
				but then \indhyp{13} ensures $\mygop < \go[\peerp]$ in $C'$.
				
				\item
				Suppose that $C.\pc{\peerp} \in \{ \refln{abrt:try:5}, \refln{abrt:try:6}, \refln{abrt:try:7} \}$ and $C.\mygop \neq C.\go[\peerp]$,
				and some process $q$ takes a step from $C$ where it changes $\go[\peerp]$ to $\mygop$.
				This scenario is impossible because $\mygop$ is non-zero (by \indhyp{12}) and
				Line~\refln{abrt:prom:6}, which is the only line of code where $q$ could possibly change $\go[\peerp]$,
				can only change $\go[\peerp]$ to 0.
				
				\item
				Suppose that $C.\pc{\peerp} \in \{ \refln{abrt:try:5}, \refln{abrt:try:6}, \refln{abrt:try:7} \} \wedge C.\csowner = (1, \peerp)$.
				Since $\peerp$ is the only process that can change the value in $\csowner$ and
				that too only at Line~\refln{abrt:exit:4}, $C.\pc{\peerp} \in \{ \refln{abrt:try:5}, \refln{abrt:try:6}, \refln{abrt:try:7} \}$ implies that 
				will continue to have the value $(1, \peerp)$ in $C'$.
			\end{itemize}
		\end{itemize}

		\item \underline{Proof that Condition~\ref{inv:abrt:cond3} holds in $C'$} \\
		We argue the correctness of the condition for the case when $\min(\minarray) = (*, \infty)$ in $C$.
		In that case the step changes the $\minarray$ so that $\min(\minarray) \neq (*, \infty)$ in $C'$.
		Since the step is by $p$, it could only be the case that $p$ took a step to write to $\minarray[p]$,
		otherwise $\minarray$ cannot change from an empty array to the one containing an element since a process writes only to its own cell in the $\minarray$.
		Such a write could happen only at Line~\refln{abrt:try:4} because at Lines~\refln{abrt:exit:1}, \refln{abrt:abort:1} $p$ could write only $(p, \infty)$.
		It follows that $\pcp = \refln{abrt:try:5}$ in $C'$, which satisfies the condition.
		\\
		\\
		Next we argue the correctness of the condition for the case when $\min(\minarray) \neq (*, \infty)$ in $C$ as below
		\begin{itemize}
			\item[Case A] $\exists q, \csowner = (1, q)$ in $C$. \\
			Suppose $\csowner = (1, q)$ in $C'$, it follows that the step didn't affect the truth value of the condition because the step was by a process $r \neq q$.
			Therefore assume $\csowner \neq (1, q)$ in $C'$.
			$\csowner$ could change from $(1, q)$ only due to the write operation by some process at Line~\refln{abrt:exit:4}.
			This process could only be $q$ itself, because if it were some process $r \neq q$, 
			then by IH:\ref{inv:abrt:cond7} and $\pc{r} = \refln{abrt:exit:4}$, $\csowner = (1, r) \neq (1, q)$ in $C$, a contradiction.
			It follows that $\pc{q} = \refln{abrt:exit:5}$ in $C'$ and the condition holds in $C'$.
			
			\item[Case B] $\forall q, \csowner \neq (1, q)$ in $C$. \\
			By IH:\ref{inv:abrt:cond2}, $\csowner = (0, \seq)$ in $C$.
			\\
			\\
			Suppose $\exists r, \csowner = (1, r)$ in $C'$.
			It follows that the execution of Line~\refln{abrt:prom:3} by some process changed the value of $\csowner$ to $(1, r)$ and the condition holds in $C'$.
			\\
			\\
			Assume $\forall q, \csowner \neq (1, q)$ in $C$.
			By IH:\ref{inv:abrt:cond3}, $\exists q,$
			$(\pc{q} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge  \go[q] \neq -1) \vee \pc{q} \in \{ \refln{abrt:try:5}, \refln{abrt:exit:5}, \refln{abrt:rec:2} \upto \refln{abrt:abort:2}, \refln{abrt:prom:1} \}$ 
			$\vee$ $(\pc{q} \in \{ \refln{abrt:prom:2}, \refln{abrt:prom:3} \} \wedge \csowner = (0, \myseq{q}))$ in $C$.
			\\
			Suppose the step changing $C$ to $C'$ was not because of $q$, the condition continues to hold in $C'$ as it held in $C$.
			\\
			Suppose the step changing $C$ to $C'$ was a crash step of $q$.
			In the case when $\pc{q} \in \{ \refln{abrt:try:5}, \refln{abrt:exit:5}, \refln{abrt:rec:2} \upto \refln{abrt:abort:2}, \refln{abrt:prom:1} \}$ 
			$\vee$ $(\pc{q} \in \{ \refln{abrt:prom:2}, \refln{abrt:prom:3} \} \wedge \csowner = (0, \myseq{q}))$ in $C$,
			by IH:\ref{inv:abrt:cond5}, $\go[q] \neq -1$ in $C$, $\pc{q} = \refln{abrt:rem:1}$ in $C'$ and $\go[q]$ remains unchanged.
			Otherwise $\pc{q} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge  \go[q] \neq -1$ in $C$, $\pc{q} = \refln{abrt:rem:1}$ in $C'$ and $\go[q]$ remains unchanged.
			In either case the step wouldn't change $\go[q]$, and the condition would continue to hold in $C'$.
			\\
			Suppose the step changing $C$ to $C'$ was a normal step of $q$.
			In that case, if $\pc{q} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge  \go[q] \neq -1$ in $C$,
			$\pc{q} \in \{ \refln{abrt:rec:1}, \refln{abrt:rec:2} \}$ in $C'$ and $\go[q] \neq -1$.
			Therefore, the condition holds in $C'$.
			Otherwise, $\pc{q} \in \{ \refln{abrt:try:5}, \refln{abrt:exit:5}, \refln{abrt:abort:2} \}$ and $q$ makes a call to $\promote{q}()$ so that changing $\pc{q}$ to $\refln{abrt:prom:1}$ and the condition being held in $C'$.
			In another case, $\pc{q} \in \{ \refln{abrt:rec:2}, \refln{abrt:abort:1} \}$ in $C$ and $\pc{q} \in \{ \refln{abrt:abort:1}, \refln{abrt:abort:2} \}$ in $C'$.
			Otherwise, $\pc{q} = \refln{abrt:prom:1}$ in $C$ and $q$ reads $\csowner$ during the step, so that $\csowner = (1, \myseq{q})$ (here $\myseq{q}$ is initialized to the second component of $\csowner$ by $q$ during the step) and $\pc{q} = \refln{abrt:prom:2}$ in $C'$.
			In another case, $\pc{q} = \refln{abrt:prom:2}$ in $C$ and it changes to $\refln{abrt:prom:3}$ in $C'$ (without modifying $\csowner$).
			In yet another case $\pc{q} = \refln{abrt:prom:3}$ in $C$ and the \casnormal\ changes $\csowner$ to $(1, \peer{q})$.
			By IH:\ref{inv:abrt:cond8}, $\peer{q} \in \procset$.
			In all these cases it follows that the condition holds in $C'$.
		\end{itemize} 
	
	
	\item \underline{Proof that Condition~\ref{inv:abrt:cond4} holds in $C'$} \\
	We first argue the correctness of the condition for the case when $\csowner \neq (1, p)$ in $C$ and $\csowner = (1, p)$ in $C'$.
	Since the step changes $\csowner \neq (1, p)$ to $(1, p)$, it happens because some process $q$ executed Line~\refln{abrt:prom:3}.
	Therefore, $\pc{q} = \refln{abrt:prom:3}$ in $C$ and changes to \refln{abrt:prom:4} because the \casnormal\ succeeds.
	Since $q$ wrote $(1, p)$ into $\csowner$ due to the \casnormal\, by an inspection of the algorithm it follows that $\peer{q} = p$ in $C$, which remains the same in $C'$.
	It follows that in $C'$ $\exists q, \pc{q} = \refln{abrt:prom:4} \wedge \peer{q} = p$. 
	Thus, the condition holds in $C'$.
	\\
	\\
	Next we argue the correctness of the condition for the case when $\csowner = (1, p)$ and $\go[p] \neq 0$ in $C$.
	By IH:\ref{inv:abrt:cond4}, $\exists q, (\pc{q} \in \{ \refln{abrt:rec:2} \upto \refln{abrt:abort:2}, \refln{abrt:prom:1} \}$ $\vee$ $(\pc{q} = \refln{abrt:prom:4} \wedge \peer{q} = p)$ 
	$\vee$ $(\pc{q} \in \{ \refln{abrt:prom:5}, \refln{abrt:prom:6} \} \wedge \peer{q} = p \wedge \mygo{q} = \go[p])$ 
	$\vee$ $(\pc{q} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1} \} \wedge \go[q] \neq -1))$
	\\
	Suppose $C$ changes to $C'$ due to a crash step of $q$.
	In that case, if $(\pc{q} \in \{ \refln{abrt:rec:2} \upto \refln{abrt:abort:2}, \refln{abrt:prom:1} \}$ $\vee$ $(\pc{q} = \refln{abrt:prom:4} \wedge \peer{q} = p)$ 
	$\vee$ $(\pc{q} \in \{ \refln{abrt:prom:5}, \refln{abrt:prom:6} \} \wedge \peer{q} = p \wedge \mygo{q} = \go[p])$,
	in all of these cases, by IH:\ref{inv:abrt:cond5}, $\go[q] \neq -1$ in $C$.
	Since the crash doesn't change $\go[q]$, it follows that $\pc{q} = \refln{abrt:rem:1}$ and $\go[q] \neq -1$ in $C'$.
	Therefore, the condition holds in $C'$.
	\\
	Suppose $C$ changes to $C'$ due to a normal step of $q$.
	In that case, if $\pc{q} \in \{ \refln{abrt:rem:1}, \refln{abrt:rec:1}, \refln{abrt:rec:2}, \refln{abrt:abort:1} \}$ in $C$, 
	it is the case that $\pc{q} \in \{ \refln{abrt:rec:1}, \refln{abrt:rec:2}, \refln{abrt:abort:2} \}$ in $C'$.
	Otherwise, a call from Line~\refln{abrt:abort:2} to $\promote{q}()$ changes $\pc{q}$ to \refln{abrt:prom:1}.
	If $\pc{q} = \refln{abrt:prom:1}$ in $C$, then since $\csowner = (1, p)$ in $C$, the step changes $\pc{q}$ to \refln{abrt:prom:4} while setting $\peer{q} = p$.
	Suppose $\pc{q} = \refln{abrt:prom:4}$ and $\peer{q} = p$ in $C$,
	and as we already assumed above that $\csowner = (1, p)$ and $\go[p] \neq 0$.
	From IH:\ref{inv:abrt:cond7}, we have $\go[p] \neq -1$ in $C$, because otherwise $\csowner \neq (1, p)$.
	It follows that the step changes $\pc{q}$ to \refln{abrt:prom:5} while setting $\mygo{q}$ to $\go[p]$.
	Since $\csowner = (1, p)$ in $C$, if $\pc{q} = \refln{abrt:prom:5}$, $\peer{q} = p$, and $\mygo{q} = \go[p]$, 
	$\pc{q}$ changes to \refln{abrt:prom:6} because the $\ifcode$ condition is met at Line~\refln{abrt:prom:5}.
	If $\pc{q} = \refln{abrt:prom:6}$, $\peer{q} = p$, and $\mygo{q} = \go[p]$ in $C$,
	the \casnormal\ at Line~\refln{abrt:prom:6} by $q$ succeeds and $\go[p]$ changes to $0$ in $C'$  thereby satisfying the condition vacuously.
	It follows that in all of the above cases the condition continues to hold in $C'$.

\end{enumerate}

Thus, by induction it follows that the invariant holds in every configuration of every run of the algorithm.
\end{proof}

